Online Resource Allocation with Samples

We study an online resource allocation problem under uncertainty about demand and about the reward of each type of demand (agents) for the resource. Even though dealing with demand uncertainty in resource allocation problems has been the topic of many papers in the literature, the challenge of not knowing rewards has been barely explored. The lack of knowledge about agents' rewards is inspired by the problem of allocating units of a new resource (e.g., newly developed vaccines or drugs) with unknown effectiveness/value. For such settings, we assume that we can \emph{test} the market before the allocation period starts. During the test period, we sample each agent in the market with probability $p$. We study how to optimally exploit the \emph{sample information} in our online resource allocation problem under adversarial arrival processes. We present an asymptotically optimal algorithm that achieves $1-\Theta(1/(p\sqrt{m}))$ competitive ratio, where $m$ is the number of available units of the resource. By characterizing an upper bound on the competitive ratio of any randomized and deterministic algorithm, we show that our competitive ratio of $1-\Theta(1/(p\sqrt{m}))$ is tight for any $p =\omega(1/\sqrt{m})$. That asymptotic optimality is possible with sample information highlights the significant advantage of running a test period for new resources. We demonstrate the efficacy of our proposed algorithm using a dataset that contains the number of COVID-19 related hospitalized patients across different age groups.

==> backup_negative_results.tex <==
%We show that 
%without using the sample information, no deterministic and randomized algorithm can obtain a CR greater than $0.5$, regardless of how large the initial  number of resources $m$ is. We further present  a  naive {protection level} algorithm that does not use the sample information and obtains a CR of at least $0.5$. This shows that the aforementioned  upper bound of $0.5$ is indeed tight and highlights the significant benefit of using the sample information.


\subsection{Negative Results: Importance of Sample Information}
In this section, we highlight the importance of the sample information by considering three settings: (i) The decision-maker does not have any sample. (ii) The decision-maker does not know the sampling probability. (iii) The samples only contain the information of the total market size, and the decision-maker cannot see how many each type agents in the sample. In each case, we give some negative results by claiming that no algorithm can have good performance. 


\subsubsection{No Sample is Accessible} {\color{red} state the setting  explicitly and say how is different from our original setting }
Without the sample information, the decision-maker is not aware the expected reward of type $i\in\{1, 2\}$ agents. Then, we claim that if we completely overlook the sample information, there is no deterministic or randomized algorithm that can achieve a CR better than $0.5$ for any value of $r_1$, $r_2$, and $m$. This immediately follows from the results in \cite{ball2009toward}. The reason is that when $r_2=0$, $r_1=1$, even if we know the reward, \cite{ball2009toward} shows that no algorithm can do better than $1/(2-\alpha) = 1/2$ for any value of $r_1, r_2,$ and $m$. 

Having this upper bound in mind,  we then present a naive algorithm (Algorithm \ref{alg:naive}) that achieves a CR of $0.5$ for any value of $r_1$, $r_2$, and $m$. In the naive algorithm, the sample information is completely overlooked. With a probability of $1/2$, the algorithm assumes that type $1$ is the type with a higher expected reward and assigns  
 a protection level of $x$ to type $1$, where $x\in \{0, 1, 2, \ldots, m\}$ is the input to the algorithm. 
 That is, the algorithm keeps accepting any type of agents until the remaining number of resources is $x$. After that, the algorithm only accepts type $1$ agents. Similarly, with a  probability of $1/2$, the algorithm assumes that type $2$ agents has a higher expected reward than type $1$ agents and then gives a protection level of  $x$ to type $2$ agents. See Algorithm \ref{alg:naive}.  
 
  
  
  
  
\begin{algorithm}[htbp]
\caption{Algorithm without Samples}
\textbf{Input:} The number of resources $m$ and protection level $x\in \{0, 1, \ldots, m\}$. 
\begin{enumerate}
  \item With probability $1/2$, we set the protection level $x$ for type $1$. In this case, we keep accepting any  agents until we have accepted $m-x$  agents. After that, we only accept  type $1$ agents. With probability $1/2$,
 set the protection level $x$ for type $2$. In this case, we keep accepting any  agents until we have accepted $m-x$  agents. After that, we reject all arriving type $1$ agents.
\end{enumerate}
\label{alg:naive}
\end{algorithm}

The following theorem shows that there exists a protection level $x$ under which  the naive algorithm that does not use the sample information can achieve a CR of at least $1/2$ for any value of $r_1$, $r_2$, and $m$.

 \begin{theorem}[Algorithm \ref{alg:naive} Achieves the Worst-Case Upper Bound $0.5$] \label{thm:naivelow}
Consider the model presented in Section \ref{sec:model}, where the expected rewards of $r_i$, $i\in \{1, 2\}$ are unknown to the decision-maker. By setting the protection level $x=m$, for any $m \ge 2$, and any $r_i \geq 0$, $i\in \{1, 2\}$, the CR of the naive algorithm (Algorithm \ref{alg:naive}) is at least $0.5$. 
\end{theorem}


To show Theorem \ref{thm:naivelow}, we observe that if $x=m$, with probability $1/2$, the naive algorithm accepts all type $1$ agents and reject all type $2$ agents, and with probability $1/2$, it accepts all type $2$ agents and reject all type $1$ agents. We can then establish a lower bound of $0.5$ on the CR of the naive algorithm by considering two cases. In the first (respectively second) case, the total number of arrivals is less (respectively greater) than or equal to $m$.

\subsubsection{Sampling Probability is Unknown} \label{subsec:unknown}

In this section, we discuss the case where $p$ is completely unknown. We analyze the case where $p$ is partially known in Section \ref{subsec:partialknown}.

Suppose that we have an estimate of the reward $r_i$
’s, $i \in \{1,2\}$. If $p$ is completely unknown, we do not have any information about the size of the market because if $p \to 0$, the real market size goes to infinity, and if $p =1$, the market size is $0$. Then, by the results in \cite{ball2009toward}, the CR cannot exceed $1/(2 - \alpha)$. This shows that without having any information about $p$, the sample information is not useful. {\color{red} state this as a result and elaborate more why we get this CR in this case. You can have a proposition.}



\subsubsection{Samples only Contain the Information of Total Market Size}

One interesting question is that: Could we obtain asymptotic optimality when the sample information only provides some information about the overall market size, instead of the market size and estimated rewards of each type? Unfortunately, the answer is no. In this case, the best attainable CR is $0.5$.  Suppose the full market size equals to $2m$, which contains $m$ type $1$ agents and $m$ type $2$ agents. Because the sample only contains the information about the total market size, we cannot estimate the reward of each type. Lacking the reward information, the best algorithm needs to accept $m/2$ type $1$ and $m/2$ type $2$ agents, which achieves a CR of $0.5$. Any other algorithm which accepts $y\ne m/2$ type $1$ agents and $z\ne m/2$ type $2$ agents fails to achieve a CR of $0.5$. This is  because if $y>z$, the algorithm has a CR less than $0.5$ when $r_1=0$, $r_2=1$. If $y<z$, the algorithm has a CR less than $0.5$ when $r_1=1$, $r_2=0$. 
{\color{red} same thing here; state a result in the form of a proposition }
